A Spatiotemporal Framework for Information Freshness in IoT Uplink Networks

Timely message delivery is a key enabler for Internet of Things (IoT) and cyber-physical systems to support wide range of context-dependent applications. Conventional time-related metrics, such as delay, fails to characterize the timeliness of the system update or to capture the freshness of information from application perspective. Age of information (AoI) is a time.evolving measure of information freshness that has received considerable attention during the past years. In the foreseen large scale and dense IoT networks, joint temporal (i.e., queue aware) and spatial (i.e., mutual interference aware) characterization of the AoI is required. In this work we provide a spatiotemporal framework that captures the peak AoI for large scale IoT uplink network. To this end, the paper quantifies the peak AoI for large scale cellular network with Bernoulli uplink traffic. Simulation results are conducted to validate the proposed model and show the effect of traffic load and decoding threshold. Insights are driven to characterize the network stability frontiers and the location-dependent performance within the network.

==> QT_anaylsis/figures/DTMC_diagram/1col/DTMC_diagram.tex <==
%% Creator: Inkscape inkscape 0.92.3, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'DTMC_diagram.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
\makeatletter%
\providecommand\color[2][]{%
	\errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
	\renewcommand\color[2][]{}%
}%
\providecommand\transparent[1]{%
	\errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
	\renewcommand\transparent[1]{}%
}%
\providecommand\rotatebox[2]{#2}%
\newcommand*\fsize{\dimexpr\f@size pt\relax}%
\newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
\ifx\svgwidth\undefined%
\setlength{\unitlength}{510.75bp}%
\ifx\svgscale\undefined%
\relax%
\else%
\setlength{\unitlength}{\unitlength * \real{\svgscale}}%
\fi%
\else%
\setlength{\unitlength}{\svgwidth}%
\fi%
\global\let\svgwidth\undefined%
\global\let\svgscale\undefined%
\makeatother%
\begin{picture}(1,0.49339207)%
\lineheight{1}%
\setlength\tabcolsep{0pt}%
\put(0,0){\includegraphics[width=\columnwidth]{QT_anaylsis/figures/DTMC_diagram/1col/DTMC_diagram.eps}}%

% column 0 
\put(0.105,0.13){$\mathcal{S}_{0}$}%
\put(0.105,0.25){\color{white}{$\mathcal{S}_{1}$}}%
\put(0.105,0.373){\color{white}{$\mathcal{S}_{2}$}}%

%column 1 
\put(0.307,0.13){$\mathcal{V}_{(1,0)}$}
\put(0.307,0.25){$\mathcal{V}_{(1,0)}$}  
\put(0.307,0.373){$\mathcal{V}_{(1,0)}$}

%column 2  
\put(0.42,0.13){$\mathcal{V}_{(0,1)}$}
\put(0.42,0.25){$\mathcal{V}_{(0,1)}$}
\put(0.42,0.373){$\mathcal{V}_{(0,1)}$}

%column 3
\put(0.535,0.13){$\mathcal{V}_{(1,1)}$}
\put(0.535,0.25){$\mathcal{V}_{(1,1)}$}
\put(0.535,0.373){$\mathcal{V}_{(1,1)}$}

%column 4
\put(0.65,0.13){$\mathcal{V}_{(2,1)}$}
\put(0.65,0.25){$\mathcal{V}_{(2,1)}$}
\put(0.65,0.373){$\mathcal{V}_{(2,1)}$}

%column 5
\put(0.77,0.13){$\mathcal{V}_{(2,2)}$}
\put(0.77,0.25){$\mathcal{V}_{(2,2)}$}
\put(0.77,0.373){$\mathcal{V}_{(2,2)}$}

% legend
\put(0.305,0.075){$\tilde{\mathbf{v}}_3$}%
\put(0.305,0.045){$\chi_3\mathbf{v}_3$}%
\put(0.305,0.018){$\bar{\chi}_3p_3$}%

\put(0.415,0.075){$\bar{\chi}_3$}%
\put(0.415,0.045){$\mathbf{V}_3$}%

\put(0.535,0.075){$\bar{\alpha}_3$}%
\put(0.535,0.045){$\alpha_3$}%

\put(0.0658556,0.011){\scriptsize{Phases}}%
\put(0.042,0.03){\rotatebox{90}{\scriptsize{Levels}}}%

\put(0.627,0.073){\scriptsize{Vacation (serving $Q_1$)}}%
\put(0.627,0.043){\scriptsize{Vacation (serving $Q_2$)}}%
\put(0.627,0.012){\scriptsize{Vacation (serving $Q_1 \rightarrow Q_2$)}}%

\put(0.823,0.073){\scriptsize{Serving $Q_3$}}%
\put(0.823,0.043){\scriptsize{Idle}}%
\put(0.32,0.19){\scriptsize{Initial vacation possible states}}%
  \end{picture}%
\endgroup%


==> QT_anaylsis/figures/VacationModelVerf/1col/VacationModelVerf.tex <==

\begin{tikzpicture}[scale=0.9]
\begin{groupplot}[group style={
	group name=myplot,
	group size= 2 by 1,  horizontal sep=2cm}, height=1.4in,width=2in]
\nextgroupplot[title={{(a)}},
scale only axis,
xmin=0,
xmax=6,
xlabel style={font=\color{white!15!black}},
xlabel={$j$},
xtick={0,1,2,3,4,5,6}, 
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={$x_{1,j}$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids]
\addplot[ycomb, color=red, dashed, line width=1.0pt, mark=otimes, mark options={solid, fill=red, red}] table[row sep=crcr] {%
	0	0.800000301068341\\
	1	0.177777844681854\\
	2	0.0197530938535393\\
	3	0.00219478820594881\\
	4	0.000243865356216534\\
	5	2.7096150690726e-05\\
	6	3.01068341008067e-06\\
};

\addplot[ycomb, color=blue, dotted, line width=2.0pt, mark=x, mark options={solid, blue}] table[row sep=crcr] {%
	0	0.800000301068341\\
	1	0.177777844681854\\
	2	0.0197530938535393\\
	3	0.00219478820594881\\
	4	0.000243865356216534\\
	5	2.70961506907261e-05\\
	6	3.01068341008067e-06\\
};


\nextgroupplot[title={{\smash{(b)}}},
scale only axis,
scale only axis,
xmin=0,
xmax=5,
xlabel style={font=\color{white!15!black}},
xlabel={$j$},
xtick={0,1,2,3,4,5}, 
ylabel={$x_{2,j}$},
ymin=0,
ymax=1,
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids]
\addplot[ycomb, color=red, dashed, line width=2.0pt, mark=*, mark options={solid, fill=red, red}] table[row sep=crcr] {%
	0	0.025105333738797\\
	1	0.0619812817198168\\
	2	0.0941059652153034\\
	3	0.146851464361824\\
	4	0.230227496730046\\
	5	0.441728458234214\\
};\addlegendentry{\cite[Ch. 9]{S.Alfa2015}}

\addplot[ycomb, color=blue, dotted, line width=2.0pt, mark=x, mark options={solid, fill=blue, blue}] table[row sep=crcr] {%
	0	0.025105333738797\\
	1	0.0619812817198169\\
	2	0.0941059652153035\\
	3	0.146851464361824\\
	4	0.230227496730046\\
	5	0.441728458234213\\
};
\addlegendentry{Proposed}

\end{groupplot}

\end{tikzpicture}

==> introduction/introduction__mostafa_Talaat_s_conflicted_copy_2019-10-16_.tex <==
% !TEX root =../integration.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% As a general rule, do not put math, special symbols or citations
% in the abstract or keywords.
\begin{abstract}
Timeliness delivery of messages is a key enabler for Internet of Things (IoT) and cyber-physical systems to support wide range of requirements from different context-dependent applications. Conventional time-related metrics, such as delay, fails to characterize the timeliness of the system updates, as they fail to capture the timeliness from the application perspective. Age of information (AoI) is a time-evolving measure of information timeliness that has received considerable attention during the past years. However, characterization of the AoI has been conducted only on the transmitters and receivers temporal scale (i.e. queues evolution), without insight on the network spatial scale (i.e., mutual interference). To this end, the paper quantifies the peak AoI for large scale IoT uplink network based on Bernoulli traffic. Simulation results are conducted to validate the proposed model and show the effect of traffic load and decoding threshold. Insights are driven to characterize the network stability frontiers and the location-dependent performance within the network.
\end{abstract}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
Age of information, spatiotemporal models, Internet of Things,  queueing theory, stochastic geometry
\end{IEEEkeywords}
% no keywords
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
%\IEEEpeerreviewmaketitle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}\label{section:introduction}
The timeliness and retainability of continuous system updates of the nodes within the system are overarching requirements among different technology segments, such as vehicular, industrial \ac{IoT} and cellular \cite{3GPP2018}. This implies continuous information update about the real-time state between a given source and its targeted destination \cite{NGMNA2016}. The proposed \ac{AoI} metric in \cite{Kaul2012} characterizes the freshness of information at the receiver and has received increasing attention in the past years. The age at a given time stamp (i.e., observation point) is defined as the current time stamp minus the time at which the observed state (or packet) was generated \cite{Yates2019}. Compared to traditional time metrics (e.g. delay and jitter), \ac{AoI} assists in achieving timely updating in a way those traditional metrics do not \cite{AoIDhillon, Ceran2018}. 

In addition, the traffic generated by the existing \ac{IoT} devices highly impact the \ac{AoI} and the overall network performance. \ac{IoT} traffic can be categorized into time and event triggered \cite{Metzger2019}. Time-triggered events that generate periodic traffic as in vehicular communications, smart grids and wireless sensor networks \cite{Palattella2016}. Moreover, event triggered traffic are dependent on external events or critical information reporting. In this paper, we consider Bernoulli-based traffic that mimic the latter scenarios to analyze the peak \ac{AoI} in uplink \ac{IoT} networks. In such segments, a central entity collects status updates from multiple nodes (e.g., sensors, vehicles and monitors) through a wireless channel. A critical challenge is how to maintain timely status updates over all the connected nodes \cite{Jiang2019}. To this end, characterizing the \ac{AoI} leads to enhancing the performance of time-critical applications.
 
\subsection{Related Work}
Based on the foreseeable large number of deployed devices \cite{Ayoub2018}, interference might hinder timely updates of a given link of interest. In order to characterize the network-wide mutual interference, stochastic geometry is a prominent framework that can be leveraged \cite{Andrews2011, Elsawy_tutorial, Haenggi2012}. Nevertheless, an underlying limiting aspect of the stochastic-geometric models is the full buffer assumption, which assumes that the transmitter always has backlogged packets to be transmitted. To account for the temporal dynamics, recent efforts have integrated queueing theory with stochastic geometry, which offers a full spatiotemporal characterization for large-scale networks \cite{Zhong2017, Gharbieh2018, Yang2019, Chisci2019, YangAoI2019}. \ac{AoI} was studied under a stochastic geometry framework in \cite{Hu2018}, where lower and upper bounds for the average \ac{AoI} were derived for an ad-hoc network. In addition, \ac{AoI} under a spatiotemporal framework has recently been investigated in \cite{YangAoI2019}, where the authors investigated different scheduling techniques to optimize the peak \ac{AoI} for an ad-hoc network. To this end, large scale spatiotemporal IoT analytical framework for peak \ac{AoI} characterization under different traffic loads is still an open research problem.

\subsection{Contributions}
Throughout this work, we provide an analytical framework to characterize peak \ac{AoI}, entailing the macroscopic and microscopic scales of uplink large scale \ac{IoT} networks. For the macroscopic aspect, tools from stochastic geometry are adopted to account for the mutual interference among active devices (i.e., location dependent). Tools from queueing theory are employed to characterize the microscopic queue evolution at each device. To track the queue status a given time stamp, a Geo/Geo/1 \ac{DTMC} is employed for each device, Geo stands for geometric inter-arrival and departure process. Expressions for the distribution of the coverage probability (i.e., meta distribution) are derived which entails the effect of the traffic characteristics. In addition, waiting time distribution and the peak \ac{AoI} are presented. To the best knowledge of the authors, this paper presents the first spatiotemporal framework that characterizes peak \ac{AoI} for an uplink \ac{IoT} network.
\subsection{Notation and Organization}
Throughout the paper, we adopt the following notation. Matrices and vectors are represented as upper-case and lower-case boldface letters ($\mathbf{A}$, $\mathbf{a}$), respectively. The indicator function is denoted as $\mathbbm{1}_{\{a\}}$ which equals 1 if the expression $a$ is true and 0 otherwise. In addition, $\mathbf{1}_m$ and $\mathbf{\mathcal{I}}_m$ denote, respectively, an all ones vector and matrix of dimension $m \times m$. In addition, identity matrix of dimension $m$ is represented via $\mathbf{I}_{m}$. The complement operator is denoted by the over-bar (i.e., $\bar{v} = 1-v$).  The notations $\mathbb{P}\{\cdot\}$ and $\mathbb{E}\{\cdot\}$ denote the probability of an event and its expectation. 

The rest of the paper is organized as follows. Section \ref{sec:system_model} provides the system model, the underlying physical and \ac{MAC} assumptions, and the peak peak \ac{AoI} characterization. Section \ref{sec:sg_analysis} shows the macroscopic inter-device interactions in terms of mutual interference. The proposed queueing model along with the microscopic intra-device interactions among the queues are presented in Section \ref{sec:QT_anaylsis}. Simulation results are presented in Section \ref{sec:simulation_results} and Section \ref{sec:Conclusion} summarizes the work.
